Full-permutation dynamical decoupling in triple-quantum-dot spin qubits

Dynamical decoupling of spin qubits in silicon can enhance fidelity and be used to extract the frequency spectra of noise processes. We demonstrate a full-permutation dynamical decoupling technique that cyclically exchanges the spins in a triple-dot qubit. This sequence not only suppresses both low frequency charge-noise- and magnetic-noise-induced errors; it also refocuses leakage errors to first order, which is particularly interesting for encoded exchange-only qubits. For a specific construction, which we call NZ1y, the qubit is isolated from error sources to such a degree that we measure a remarkable exchange pulse error of $5\times10^{-5}$. This sequence maintains a quantum state for roughly 18,000 exchange pulses, extending the qubit coherence from $T_2^*=2~\mu$s to $T_2 = 720~\mu$s. We experimentally validate an error model that includes $1/f$ charge noise and $1/f$ magnetic noise in two ways: by direct exchange-qubit simulation, and by integration of the assumed noise spectra with derived filter functions, both of which reproduce the measured error and leakage with respect to changing the repetition rate.

==> frontmatter.tex <==
\RequirePackage{varioref}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{graphicx}
\RequirePackage{color}

% These are commands to add colorful inline comments of different types.
% They can all be turned off at once by setting the boolean "ShowComments' to false in the preamble.

\ifthenelse{\boolean{ShowComments}}%
{
	\newcommand{\ColorComment}[3]{%
		{\colorbox{#1}{\color{white}   \textsf{\textbf{#2}}} \textcolor{#1}{#3}}}%  Colorful box, initials, phrase 
	\newcommand{\nyacite}[1]{[#1]}% not yet a cite
}%
{
	\newcommand{\ColorComment}[3]{}%  Do nothing at all
	\newcommand{\nyacite}[1]{}% not yet a cite -- do nothing
}%

% Assign special colors to kinds of comments.
\definecolor{storyboardcolor}{rgb}{1,0,1}
\newcommand{\storyboard}[1]{\ColorComment{storyboardcolor}{Outline}{#1}}
\definecolor{tdlcolor}{rgb}{0,0.7,0}
\newcommand{\tdl}[1]{\ColorComment{tdlcolor}{tdl}{\textsf{#1}}}
\definecolor{tdltextcolor}{rgb}{0,0.4,0}
\newcommand{\tdlsuggests}[1]{%
	\ColorComment{tdltextcolor}{PROPOSED:}{\textsf{#1}}}

\definecolor{tbcolor}{rgb}{1.0,0,0}
\newcommand{\tb}[1]{\ColorComment{tbcolor}{tb}{\textsf{#1}}}

\definecolor{bscolor}{rgb}{0.4,0.2,0.8}
\newcommand{\bsun}[1]{\ColorComment{bscolor}{bs}{\textsf{#1}}}

\definecolor{jzbcolor}{rgb}{0.1,0.2,0.9}
\newcommand{\jzb}[1]{\ColorComment{jzbcolor}{jzb}{\textsf{#1}}}

\definecolor{sjwcolor}{rgb}{.5,.5,0}
\newcommand{\sjw}[1]{\ColorComment{sjwcolor}{sjw}{\textsf{#1}}}

\definecolor{mtrcolor}{rgb}{1,0.4,0}
\newcommand{\mtr}[1]{\ColorComment{mtrcolor}{mtr}{\textsf{#1}}}

% A pure comment, meaning don't typeset the argument at all
\newcommand{\com}[1]{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% To save typing on all math commands
\newcommand{\mathcommand}[3][0]{\newcommand{#2}[#1]{\ensuremath{#3}}}
%%%%%%%%%%%%%%%%% Some common vectors
\renewcommand{\vec}[1]{\ensuremath{\text{\textbf{#1}}}} % Simply a bold charactor.

\newcommand{\isotope}[2]{\ensuremath{^{#2}\text{#1}}}
\newcommand{\Si}{\isotope{Si}{29}}
\newcommand{\Ge}{\isotope{Ge}{73}}
\newcommand{\CPn}{CP$n$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Equation Environments
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Some common colors
\newcommand{\green}{\textcolor[rgb]{0,0.4,0}}
\newcommand{\purple}{\textcolor[rgb]{0.8,0.2,0.6}} %Chosen to match standard Powerpoint colors
\newcommand{\blue}{\textcolor[rgb]{0,0,0.7}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\teal}{\textcolor[rgb]{0,0.4,0.3}}
\newcommand{\darkyellow}{\textcolor[rgb]{0.8,0.6,0}}
\newcommand{\orange}{\textcolor[rgb]{1,0.4,0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text subscripting
\newcommand{\ts}[2]{{#1}_{\textnormal{#2}}} %A math symbol with a text subscript
\newcommand{\tsc}[2]{{#1}_{\textsc{\lowercase{#2}}}} %A math symbol with a text subscript

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Trace
\newcommand{\Tr}[2][]{\text{Tr}_\text{#1}\left\{#2\right\}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Bra Ket notation
\mathcommand[1]{\smallket}{|#1\rangle}
\mathcommand[1]{\smallbra}{\langle #1|}
\mathcommand[1]{\bigket}{\bigl|#1\bigr\rangle}
\mathcommand[1]{\bigbra}{\bigl\langle #1\bigr|}
\mathcommand[1]{\biggket}{\biggl|#1\biggr\rangle}
\mathcommand[1]{\biggbra}{\biggl\langle #1\biggr|}
\mathcommand[1]{\ket}{\left| #1 \right\rangle}  %a Ket
\mathcommand[1]{\lket}{\bigl| #1 \bigr)}  %a Liouville Ket
\mathcommand[1]{\bra}{\left\langle #1 \right|}  %a Bra
\mathcommand[1]{\lbra}{\bigl( #1 \bigr|}  %a Bra
\newcommand{\ketbra}[2]{\left| #1 \right\rangle\!\!\left\langle #2
\right|} %an outer product
\newcommand{\braket}[2]{\left\langle #1 |#2\right\rangle} %an inner product
\newcommand{\bigbraket}[2]{\bigl\langle #1 \bigl| #2 \bigr\rangle} %an inner product
\newcommand{\biggbraket}[2]{\biggl\langle #1 \biggl| #2 \biggr\rangle} %an inner product
\newcommand{\bigketbra}[2]{\bigl| #1 \bigr\rangle\!\bigl\langle #2
\bigr|} %an outer product
\newcommand{\lbraket}[2]{\bigl( #1 \bigl| #2 \bigr)} %an inner product
\newcommand{\lketbra}[2]{\bigl| #1 \bigr)\!\!\bigl( #2
\bigr|} %an outer product
\newcommand{\sizedlbraket}[2]{\left.\left( #1 \left| #2 \right)\right.\right.} %an inner product
\newcommand{\biglbraket}[2]{\biggl(#1\biggl|#2\biggr)}
    % This one (above) scales to the right size, but:
    % works only if bra is smaller than ket
    % If something else is needed, define \rbraket
    % These Always make big delimiters
\newcommand{\bbraket}[2]{\biggl\langle #1 \biggm| #2 \biggr\rangle}
\mathcommand[1]{\bbra}{\biggl\langle #1 \biggr|}
\mathcommand[1]{\bket}{\biggl| #1 \biggr\rangle}
\newcommand{\gsket}{\ket{\Omega}}  %Ground state
\newcommand{\gsbra}{\bra{\Omega}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Referencing Equations
% Uses package varioref
%\renewcommand{\reftextcurrent}{}
\newcommand{\refeq}[1]{Eq.~\eqref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\reffig}[1]{Fig.~\ref{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Wigner-Eckart stuff
\newcommand{\redmat}[3]{\bra{#1}\!|#2|\!\ket{#3}}
\newcommand{\bigredmat}[3]{\bigbra{#1}\!\bigl|#2\bigr|\!\bigket{#3}}
\newcommand{\vecirrep}[1]{\hat{\vec{#1}}}
\newcommand{\sixj}[6]{
\left\{\!\begin{array}{lcr}#1&#2&#3\\
                           #4&#5&#6\end{array}\!\right\}}
                           



